Measuring Visual Generalization in Continuous Control from Pixels

Self-supervised learning and data augmentation have significantly reduced the performance gap between state and image-based reinforcement learning agents in continuous control tasks. However, it is still unclear whether current techniques can face a variety of visual conditions required by real-world environments. We propose a challenging benchmark that tests agents' visual generalization by adding graphical variety to existing continuous control domains. Our empirical analysis shows that current methods struggle to generalize across a diverse set of visual changes, and we examine the specific factors of variation that make these tasks difficult. We find that data augmentation techniques outperform self-supervised learning approaches and that more significant image transformations provide better visual generalization \footnote{The benchmark and our augmented actor-critic implementation are open-sourced @ https://github.com/QData/dmc_remastered)

==> makefile <==
RCSFLAGS= -l
MAIN= paper
FINAL= final
TEXPARTS= \
    000abstract.tex \
    010introduction.tex \
    020background.tex \
    030method.tex \
    040experiment.tex \
    060conclusion.tex \
    070appendix.tex \
    dfn.tex

BIBPARTS= BIB/*.bib
# POSTSCRIPT= dvips -P cmz -t letter  #dvips -f
# FIGPARTS= FIG/*.eps  FIG/*.pdf FIG/*.fig FIG/*.png
FIGPARTS= FIG/*.png FIG/*.dia FIG-TIKZ/*.tex
STYPARTS= sig-alternate.cls
# algorithm2e.sty \
#	  algorithmic.sty \
#	  url.sty \
#	  xspace.sty
OTHER= mkfinal.pl makefile README.txt
ALL= $(MAIN).tex $(TEXPARTS) $(BIBPARTS) $(FIGPARTS) $(STYPARTS) $(OTHER)

$(MAIN).pdf: $(MAIN).tex $(TEXPARTS) 
	pdflatex $(MAIN).tex
	bibtex $(MAIN)
	pdflatex $(MAIN).tex
	pdflatex $(MAIN).tex

final: $(FINAL).pdf

$(FINAL).pdf: $(MAIN).tex mkfinal.pl
	mkfinal.pl $(MAIN).tex > $(FINAL).tex
	pdflatex $(FINAL).tex
	bibtex $(FINAL)
	pdflatex $(FINAL).tex
	pdflatex $(FINAL).tex

try: $(MAIN).tex
	pdflatex $(MAIN)


clean:
	\rm -f *.dvi $(MAIN).ps *.bbl *.aux *.log *.blg *.toc all.tar* uu \
	*~ *.bak *.lbl *.brf

spotless: clean
	\rm -f $(MAIN).ps $(MAIN).pdf
	\rm -f $(FINAL).*
	\rm -rf TST

all.tar:
	tar cvfh all.tar $(ALL)


